Enhance Modality Robustness in Text-Centric Multimodal Alignment with Adversarial Prompting

Converting different modalities into generalized text, which then serves as input prompts for large language models (LLMs), is a common approach for aligning multimodal models, particularly when pairwise data is limited. Text-centric alignment method leverages the unique properties of text as a modality space, transforming diverse inputs into a unified textual representation, thereby enabling downstream models to effectively interpret various modal inputs. This study evaluates the quality and robustness of multimodal representations in the face of noise imperfections, dynamic input order permutations, and missing modalities, revealing that current text-centric alignment methods can compromise downstream robustness. To address this issue, we propose a new text-centric adversarial training approach that significantly enhances robustness compared to traditional robust training methods and pre-trained multimodal foundation models. Our findings underscore the potential of this approach to improve the robustness and adaptability of multimodal representations, offering a promising solution for dynamic and real-world applications.

==> AnonymousSubmission/LaTeX/main_result.tex <==
% \begin{figure*}[t]
% \centering
%   \centering
%   \includegraphics[width=\linewidth]{Figs/result.png}
%   \caption{Results}
%   \label{fig:exp:results}
% \end{figure*}










% \begin{figure*}[t]
% \centering

% % First column of figures
% \begin{subfigure}[t]{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/acc_all.pdf}
%   \caption{Acc - All}
%   \label{fig:acc_all}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/drop_all.pdf}
%   \caption{Drop - All}
%   \label{fig:drop_all}
% \end{subfigure}

% %\vspace{0.5cm}

% % Second column of figures
% \begin{subfigure}[t]{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/acc_image.pdf}
%   \caption{Acc - Image}
%   \label{fig:acc_image}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/drop_image.pdf}
%   \caption{Drop - Image}
%   \label{fig:drop_image}
% \end{subfigure}

% %\vspace{0.5cm}

% % Third column of figures
% \begin{subfigure}[t]{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/acc_text.pdf}
%   \caption{Acc - Text}
%   \label{fig:acc_text}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/drop_text.pdf}
%   \caption{Drop - Text}
%   \label{fig:drop_text}
% \end{subfigure}

% %\vspace{0.5cm}

% % Fourth column of figures
% \begin{subfigure}[t]{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/acc_table.pdf}
%   \caption{Acc - Table}
%   \label{fig:acc_table}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\linewidth}
%   \centering
%   \includegraphics[width=\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/drop_table.pdf}
%   \caption{Drop - Table}
%   \label{fig:drop_table}
% \end{subfigure}

% \caption{Results}
% \label{fig:exp:results}
% \end{figure*}











% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.33\linewidth]{Figs/main/all_main_acc.pdf}
%   \includegraphics[width=0.33\linewidth]{Figs/main/all_main_drop.pdf}
%   \hfill
%   \includegraphics[width=0.33\linewidth]{Figs/main/all_main_acc.pdf}
%   \includegraphics[width=0.33\linewidth]{Figs/main/all_main_drop.pdf}
%   \hfill
%   \includegraphics[width=0.33\linewidth]{Figs/main/all_main_acc.pdf}
%   \includegraphics[width=0.33\linewidth]{Figs/main/all_main_drop.pdf}
%   \caption{To evaluate robustness with noise applied to all three modalities, we analyzed accuracy (left) and drop ratio (right). Both metrics indicate that the text-centric method demonstrates stronger robustness and better resistance to noise compared to other baselines as the noise level increases.}
%   \label{fig:acc_drop_all}
% \end{figure*}

% Second row of figures
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=1.0\linewidth]{Figs/main/specific_main_drop.pdf}
%   \caption{Drop ratio when noise is applied to modalities separately - Image (left) and Table (center) and Text (right). Text-centric methods outperforms all baselines and remain nearly no declined as the noise level increase.}
%   \label{fig:acc_drop_image}
% \end{figure*}

% % Third row of figures
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.48\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/acc_text.pdf}
%   \includegraphics[width=0.48\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/drop_text.pdf}
%   \caption{Acc - Text (left) and Drop - Text (right)}
%   \label{fig:acc_drop_text}
% \end{figure*}

% % Fourth row of figures
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=0.48\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/acc_table.pdf}
%   \includegraphics[width=0.48\linewidth, trim={0 15cm 0 0}, clip]{Figs/main/drop_table.pdf}
%   \caption{Acc - Table (left) and Drop - Table (right)}
%   \label{fig:acc_drop_table}
% \end{figure*}
